Geometry of canonical bases and mirror symmetry

A decorated surface S is a surface with a finite set of special points on the boundary, considered modulo isotopy. Let G be a split reductive group. A pair (G, S) gives rise to a moduli space A(G, S), closely related to the space of G-local systems on S. It has a positive structure. So the set of its integral tropical points is defined. We introduce a rational positive function W on A(G, S), the potential. The condition that its tropicalisation is non-negative determines its subset. For SL(2), we recover the set of integral laminations on S. We prove that when S is a disc with n special points on the boundary, this set parametrises top dimensional components of the convolution varieties. Thus, via geometric Satake correspondence, they provide a canonical basis in tensor product invariants of irreducible modules for the Langlands dual group. When G=GL(m), n=3, there is a special coordinate system on A(G,S). We show that it identifies our set with the set of with Knutson-Tao's hives. Our result generalises a theorem of Kamnitzer, who used hives to parametrise top components of convolution varieties for GL(m), n=3. For n>3, we prove Kamnitzer's conjecture. We define canonical bases in tensor products, generalizing the Mirkovic-Vilonen basis in a single representation. We prove that for any S, the set of positive integral tropical points of A(G, S) parametrise top components in a new space, surface affine Grasmannian. We view W as a potential for Landau-Ginzburg model on A(G,S). We conjecture that the pair (A(G,S), W) is the mirror dual to the moduli space of local systems on S for the Langlands dual group. In a special case, we recover Givental's description of the quantum cohomology connection for flag varieties.

==> surface.tex <==
%\section{The potential ${\cal W}$ and Weyl group actions on the space ${\cal A}_{{\rm G},   S}$} \la{sec11}
\section{The Weyl group actions on the space ${\cal X}_{\G, S}$ are positive} \la{sec10n}
\subsection {The moduli space ${\cal X}_{\G, S}$} 
\la{xmodsp}
In Section \ref{sec10n}, $\G$ is a split semisimple algebraic group over $\Q$ with trivial center. 
%Recall the decorated surface $S$ and its dual surface $\ast S$ in Section \ref{sec11}.
Given a right ${\rm G}$-local system ${\cal L}$ on $S$, there is the associated flag  bundle ${\cal L}_{\cal B}:={\cal L}\times_{\G}{\cal B}$.

\bd[\cite{FG1}]
The moduli space ${\cal X}_{{\rm G},   S}$  parametrizes 
pairs $({\cal L}, \beta)$ where ${\cal L}$ is a ${\G}$-local system on $S$, and 
$\beta$ a flat section of the restriction of ${\cal L}_{\cal B}$ 
 to  the punctured boundary  $\widehat \partial (\ast S)$. 
\ed
%Note that $s_{\G}$ is trivial. There is no need to consider the ``twisted" $\G$-local systems. 

If $S$ is a disk $D_n$ with $n$-special points on its boundary, then ${\cal X}_{\G,D_n}={\rm Conf}_n({\cal B})$.

We briefly recall the positive structure of ${\cal X}_{\G, S}$ introduced in {\it loc.cit.}
Let $T$ be an ideal triangulation of $S$, ${\cal T}$ the set of the triangles of $T$, and 
${\cal E}_{\rm int}$ the set of the internal edges of $T$.  There is a birational map 
\be
\displaystyle{
\pi_{T}: {\cal X}_{\G, S}\lra \Pi_{t\in {\cal T}}{\rm Conf}_3({\cal B})\times {\Pi}_{e\in {\cal E}_{\rm int}}{\rm H}}.
\ee
The map to the first factor is defined by restricting ${\cal X}_{\G, S}$ to the triangles $t\in {\cal T}$.
Recall the basic invariants in Section \ref{sec2.3.2}.
If $S=D_4$, then the map to second factor is 
$$
p_{13}:
{\rm Conf}_4({\cal B})\lra {\rm H},~~(\B_1, \B_2,\B_3, \B_4)\lms \frac{\alpha(\A_1, \A_2)}{\alpha(\A_3, \A_2)}\frac{\alpha(\A_3,\A_4)}{\alpha(\A_1, \A_4)}, ~~~\mbox{where $\A_i\in {\cal A}$ and $\pi(\A_i)=\B_i$}.
$$
In general, one can go to a finite cover of $S$ if needed, and construct a similar map from ${\cal X}_{\G, S}$ to ${\Pi}_{e \in {\cal E}_{\rm int}}{\rm H}$.
Note that both ${\rm Conf}_3({\cal B})$ and ${\Pi}_{e \in {\cal E}_{\rm int}}{\rm H}$ admit  natural positive structures. The positive structure on ${\cal X}_{\G, S}$ is defined such that $\pi_{T}$ is a positive birational isomorphism.
It is proved in {\it loc.cit} that the positive structure on ${\cal X}_{\G, S}$ is independent of the  triangulation $T$ chosen.


\vskip 2mm

Let $g\in \G$ be a regular semisimple element. It is well known that the set ${\bf B}_{g}$ of Borel subgroups containing $g$ is a $W$-torsor. 
Let ${\rm C}$ be a boundary circle of $S$. Given a generic pair $({\cal L}, {\beta})\in{\cal X}_{\G, S}$, 
the monodromy around ${\rm C}$ preserve the flat section ${\beta}|_{{\rm C}}$ restricted to ${\rm C}$. In particular, if we trivialize ${\cal L}$ at the fiber ${\cal L}_x$ over a point $x\in {\rm C}$, then the flat section ${\beta}|_{{\rm C}}$ becomes a Borel subgroup containing the monodromy $g$. This defines a Weyl group action on ${\cal X}_{\G, S}$.
 
\bd [${\it loc.cit}$]
For each boundary circle ${\rm C}$ of $S$, there is a rational Weyl group action on ${\cal X}_{\G,S}$ by 
altering the flat section over ${\rm C}$. 
\ed

In the rest of this Section, we prove 

\bt \la{13.5.4.11115h}
The Weyl group acts on ${\cal X}_{\G, S}$ by positive birational isomorphisms.
\et


\subsection{A positive Weyl group action on ${\rm Conf}({\cal A},{\cal A},{\cal B})$}

\la{sec7.01h}

The $\G$-orbits of ${\cal B}\times{\cal B}$ are parametrized by the Weyl group. Two flags $\B_1,\B_2$ are called of distance $w$, denoted by  $\B_1\stackrel{w}{\ra}\B_2$, if $\{\B_1,\B_2\}$ belongs to the orbit parametrized by $w$.
Let us fix a flag $\B^-$. Let ${\cal B}_w$ be the set of flags $\B'$ 
such that $\B^-\stackrel{w}{\ra}\B'$. Then we have 
$
{\cal B}=\bigsqcup_{w\in W}{\cal B}_w.
$ 
 In particular,  the flags $x_i(c)\cdot \B^{-}$ ($c\in {\Bbb G}_m$) are in ${\cal B}_{s_i}$.
 
Let $g\in {\rm G}$ be a regular semisimple element. As stated in Section \ref{xmodsp}, the set  ${\bf B}_g$ of  Borel subgroups 
containing $g$ is a $W$-torsor. 
For example,  if $b\in \B^{-}$ is  a regular semisimple element, then in each cell ${\cal B}_w$, there exists a unique Borel subgroup containing $b$.

\vskip 2mm

Let ${\bf x}=\{\A_1, \A_2, \B_3\}\in {\cal A\times A\times B}$ be  a generic point. There is a unique $b_{\bf x}\in \B_3$ taking $\A_1$ to $\A_2$. Since the subset of regular semisimple elements in $\G$ is Zariski open, we can assume that $b_{\bf x}$ is regular semisimple. Let  $\B_{{\bf x}}^w$ be the unique Borel subgroup containing $b_{\bf x}$ such that $\B_3\stackrel{w}{\ra}\B_{\bf x}^{w}$. 
Set 
$$w({\bf x}):=\{\A_1, \A_2, \B_{\bf x}^{w}\}.$$ 
It defines a rational Weyl group action on ${\cal A\times A\times B}$. 
Such an action commutes with the $\G$-diagonal action. 
Thus it descends to an action on ${\rm Conf}({\cal A},{\cal A}, {\cal B})$. 

\bt \la{13.5.4.1211h}
The Weyl group action on ${\rm Conf}({\cal A, A, B})$ is a  positive action. 
\et


First we recall the following basic facts.

\vskip 1mm

1) The set of conjugacy classes of parabolic subgroups of $\G$ is in bijection with the subsets of $I$. Let $i\in I$. Denote by ${\cal P}_i$ the space of parabolic subgroups corresponding to $\{i\}$. 
For any  Borel subgroup $\B$, there is a unique  ${\rm P}\in {\cal P}_i$ containing $\B$. Denote by ${\cal B}_{\rm P}$ the space of Borel subgroups contained in ${\rm P}$. Then ${\cal B}_{\rm P}\stackrel{\sim}{=}\P^1$. It 
 consists of $\B$ and Borel subgroups which are of distance $s_i$ to $\B$. 


\vskip 1mm

2) Let ${\P}_*:=\P^1-\{y_1, y_2\}$ be the projective line without two points. 
 Consider the cross ratio
$$
r(z_1,z_2; y_1, y_2)=\frac{(z_1-y_1)(z_2-y_2)}{(z_1-y_2)(z_2-y_1)}, ~~~~\mbox{where } z_1, z_2\in {\P}_*.
$$
Since $r(z_1,z_2;y_1, y_2)r(z_2, z_3;y_1, y_2)=r(z_1, z_3; y_1, y_2)$,
it gives rise to a ${\Bbb G}_m$-action on $\P_*$
 such that
$$
\forall c\in {\Bbb G}_m, \forall z\in {\P}_*,~~~~
r(z, c\cdot z; y_1, y_2)=c.
$$
Let ${\rm P}\in {\cal P}_i$. Since ${\cal B}_{\rm P}\stackrel{\sim}{=}{\P}^1$, each pair of distinct Borel subgroups contained in  ${\rm P}$ will give rise to a rational ${\Bbb G}_m$-action on ${\cal B}_{\rm P}$.

\vskip 1mm

3) Let $w=w_1w_2$ be such that $l(w)=l(w_1)+l(w_2)$. For any pair $\B\stackrel{w}{\ra}\B'$, there is a unique Borel subgroup $\B_1$ such that $\B\stackrel{w_1}{\ra}\B_1\stackrel{w_2}{\ra}\B'$. In particular, if $\{\B, \B'\}$ is of distance $w_0$, then each reduced word ${\bf i}=(i_1,\ldots, i_m)$ for $w_0$ gives rise to a unique chain
$$
\B=\B_0\stackrel{s_{i_1}}{\lra}\B_1\stackrel{s_{i_2}}{\lra}\ldots \stackrel{s_{i_m}}{\lra}\B_m=\B'.
$$ 
Let $\A\in {\cal A}$ be a generic decorated flag. Set $a_k:=\chi(u_{\B_{{k-1}}, \B_{k}}^\A)$. It is easy to see that $u_{\B_{{k-1}}, \B_{k}}^\A=x_{i_k}(a_k)$. It recovers Lusztig's coordinate: $u_{\B, \B'}^{\A}=x_{i_1}(a_1)\ldots x_{i_m}(a_m)$.

\vskip 2mm

Let ${\bf x}=\{\A_1, \A_2, \B_3\}\in {\cal A\times A\times B}$ be  a generic point. 
Let $i\in I$. Set $\B_1'$, $\B_2'$ such that
\be \la{13.4.22.955h}
\B_3\stackrel{s_i}{\lra}\B_k'\stackrel{s_iw_0}{\lra}\pi(\A_k),~~~~ k=1,2.
\ee
Let ${\rm P}\in {\cal P}_i$ contain  $\B_3$. Note that $\B_1', \B_2'\in{\cal B}_{\rm P}$. 
They give rise to a ${\Bbb G}_m$-action on ${\cal B}_{\rm P}$.
Denote by $c\cdot \B_3$ the image of $\B_3$ under the action of $c\in {\Bbb G}_m$. Set
\be \la{13.4.22.2108h}
e_i^c({\bf x}):=\{\A_1, \A_2, c\cdot \B_3\}.
\ee
It defines a rational ${\Bbb G}_m$-action on ${\cal A\times A\times B}$.
There is a unique $u_1'$ in the stabilizer of $\A_1$ transporting $\B_3$ to $\B_2'$. There is a unique $u_2'$ in the stabilizer of $\A_2$ transporting $\B_1'$ to $\B_3$.  Set 
\be \la{13.6.8.12.41h}
l_i({\bf x})=\chi_{\A_1}(u_1'),~~~~~
r_i({\bf x})=\chi_{\A_2}(u_2').
\ee
Since $e_i^\ast$, $l_i$, $r_i$ commute with the $\G$-diagonal action, we can descend them to  ${\rm Conf}({\cal A},{\cal A}, {\cal B}).$

\vskip 3mm


Theorem \ref{13.5.4.1211h} is a direct consequence of the following Lemmas.

\bl \la{13.6.9.1548h}
The functions $l_i, r_i$ are positive functions. The action $e_i^{\ast}$ is a positive action. 
\el

\begin{proof}
Let ${\bf i}=(i_1,\ldots, i_m)$ be a reduced word for $w_0$ which starts from $i_1=i$. 
Let ${x}=(\A_1, \A_2, \B_3)$ be a generic configuration.
We associate to $x$ two chains of Borel subgroups: 
\be \la{13.4.22.1354h}
\B_3=\B_0'\stackrel{s_{i_1}}{\lra}\B_1'\stackrel{s_{i_2}}{\lra}\ldots \stackrel{s_{i_m}}{\lra}\B_{m}'=\pi(\A_2),~~~~~\pi(\A_1)=\B_m''\stackrel{s_{i_m}}{\lra}\ldots\stackrel{s_{i_{2}}}{\lra}\B_1'' \stackrel{s_{i_1}}{\lra}\B_0''=\B_3.
\ee
Set
\be \la{13.5.5.1122h}
h:=h_{\A_1, \A_2}\in {\rm H},~~~~
a_k:=\chi(u_{\B_{k-1}',\B_{k}'}^{\A_1}),~b_k:=\chi(u_{\B_k'', \B_{k-1}''}^{\A_2}).
\ee
Recall the left and right functions ${\cal L}_i$ and ${\cal R}_i$.  By definition,
\be \la{8.13.4.4h}
l_i(x)={\cal L}_i(u_{\rm B_3, B_2}^{\rm A_1})=a_1,~~~~~ 
r_i(x)={\cal R}_i(u_{\rm B_1, B_3}^{\rm A_2})=b_1, 
\ee
The positivity of $l_i$, $r_i$ follows. By  definition, we get
\be \la{13.4.22.1452h}
l_i(e_i^c({x}))=cl_i ({x})=ca_1,~~~~ 
r_i(e_i^c({ x}))=r_i({ x})/c=b_1/c.
\ee
Recall the  birational isomorphism
$p:{\rm Conf}({\cal A},{\cal A},{\cal B})\ra{\B}^{-}$ mapping $(\A_1,\A_2,\B_3)$ to $b_{\B_3}^{\A_1,\A_2}.$
Using \eqref{13.4.22.1354h}\eqref{13.5.5.1122h}, we get a decomposition
\be \la{8.15.3.0h}
p({x})=x_{i_1}(a_1)\ldots x_{i_m}(a_m)h\overline{w}_0x_{i_m}(b_m)\ldots x_{i_1}(b_1).
\ee
Note that the action $e_i^c $ only changes $\B_0'$, $\B_0''$ to $c\cdot \B_3$ in \eqref{13.4.22.1354h}. Combining with  \eqref{13.4.22.1452h}, we get
\be \la{13.4.22.1550h}
p(e_i^c( x))=x_{i_1}(ca_1)\ldots x_{i_m}(a_m)h\overline{w}_0x_{i_m}(b_m)\ldots x_{i_1}(b_1/c).
\ee
It multiplies the first term by $c$, divides the last term by $c$, and keeps the rest intact. Thus it defines a positive rational ${\Bbb G}_m$-action on $\B^-$.  
Since $p$ is a positive birational isomorphism,  the positivity of the action $e_i^\ast $ follows.
\end{proof}


\bl Let $i\in I$. For each generic $ x\in {\rm Conf}({\cal A},{\cal A},{\cal B})$, we have
\be
s_i(x)=e_i^{c_i}(x),~~~~~~\mbox{where } c_i=r_{i}(x)/l_{i}(x). 
\ee
\el



\begin{proof}
Note that $x$
has a representative
${\bf x}=\{\U, p(x)\cdot \U, \B^{-}\}\in {\cal A}\times {\cal A}\times{\cal B}$, where $p(x)$ has a decomposition \eqref{8.15.3.0h}.
So $c_{i}=b_1/a_1$.
Set $u:=x_{i}(a_1-b_1)$.  By \eqref{13.4.22.1550h},
$$
p\big(e_{i}^{c_{i}}(x)\big) ={\rm Ad}_{u^{-1}}(p(x))= x_{i_1}(b_1)\ldots x_{i_m}(a_m)h\overline{w}_0x_{i_m}(b_m)\ldots x_{i_1}(a_1)
\in \B^{-}. 
$$
Therefore $p(x)\in u\cdot \B^{-}$. Note that $\B^{-}\stackrel{s_{i}}{\ra}  u\cdot\B^{-}$. Then  $s_{i}({\bf x})=\{\U, p(x)\cdot \U, u\cdot \B^-\}$. Therefore
$$
s_{i}(x)=(\U, p(x)\cdot \U, u\cdot \B^-)=(\U, {\rm Ad}_{u^{-1}}(p(x))\cdot \U, \B^{-})=e_{i}^{c_{i}}(x).
$$ 
\end{proof}

There is a natural projection ${\rm Conf}({\cal A}^{n+1}, {\cal B})\ra {\rm Conf}({\cal A, A, B})$ sending $(\A_1,\ldots, \A_{n+1}, \B)$ to $(\A_1, \A_{n+1}, \B)$. The Weyl group action on ${\rm Conf}({\cal A, A, B})$ induces an action on ${\rm Conf}({\cal A}^{n+1}, {\cal B})$. 
The following Corollary is clear.
\bc \la{13.5.6.953h}
The induced Weyl group action on ${\rm Conf}({\cal A}^{n+1}, {\cal B})$ is a positive action.
\ec

\subsection{Proof of Theorem \ref{13.5.4.11115h}} \la{sec11.1.2}

Let us shrink all holes without special points on $S$ into punctures, getting a homotopy equivalent surface denoted again by $S$. 
Let $D_1^*$ be a punctured disk with one special point on its boundary. 
Let ${\cal L}_{\G, D^*_1}$ be the moduli space parametrizing the triples $({\cal L}, {\alpha}, \beta)$ where ${\cal L}$ is a $\G$-local system on $D^*_1$, $\alpha$ is flat section of ${\cal L}_{\cal A}$ restricted to the neighbor of the special point, and $\beta$ is a flat section of ${\cal L}_{\cal B}$ restricted to the loop around the puncture.

Taking a triangle with two $\A$-vertices and one $\B$-vertex, see  Fig \ref{tpm16}, 
and gluing it as shown, we obtain a birational isomorphism: 
 \be \la{biriso}
{\rm Conf}({\cal A},{\cal A}, {\cal B}) \stackrel{\sim}{=} {\cal L}_{\G, D^*_1}.
\ee
\begin{figure}[ht]
%\epsfxsize250pt
\centerline{\epsfbox{tpm16.eps}}
\caption{Birational isomorphism of  moduli spaces ${\rm Conf}({\cal A},{\cal A}, {\cal B}) \sim {\cal L}_{\G, D^*_1}$.}
\label{tpm16}
\end{figure}
Let us elaborate \eqref{biriso}. 
Let $\{\A_1, \A_2, \B\}$ be a generic triple.
Let $b\in \G$ be the unique element such that  $b\cdot\{\B, \A_1\} = \{\B, \A_2\}$. 
Then $b \in \B$. 
We glue the sides $\{\B, \A_1\}$ and $\{\B, \A_2\}$, matching the flags. 
We get a disc with a special point $s$ and a puncture $p$. 
There is a $\G$-local system on the punctured disc, trivialized over the segment connecting the 
points $s$ and $p$ (the dashed segment in the disc on Fig \ref{tpm16}),  
with the clockwise monodromy $b$. It has an invariant flag at the puncture -- the flag $\B$. 
It also has a decorated flag at the special point $s$. Another configuration 
$\{g\A_1, g\A_2, g\B\}$ provides an isomorphic object. 
Thus it provides a rational map ${\rm Conf}({\cal A}, {\cal A}, {\cal B})\to {\cal L}_{\G, D_1^*}$. 
Its inverse map is obtained by cutting  $D_1^*$ along this dashed segment.

Note that there is a natural projection ${\cal L}_{\G, D_1^*}\ra {\cal X}_{\G, D_1^*}$.
Composing with the isomorphism \eqref{biriso}, we obtain a positive rational dominant map $p: {\rm Conf}({\cal A}, {\cal A}, {\cal B})\ra {\cal X}_{\G, D_1^*}$.
By definition, it commutes with the Weyl group actions on both spaces.
 It is easy to show that a rational function $f$ of ${\cal X}_{\G, D_1^*}$ is positive if and only if the function $p^*(f)$ of ${\rm Conf}({\cal A}, {\cal A}, {\cal B})$ is positive. 
By Theorem \ref{13.5.4.1211h}, the $W$-action on  ${\cal X}_{\G, D^*_1}$ is positive.


Let $D_n^*$ be a punctured disk with $n$ special points on its boundary. Similarly the $W$-action on ${\cal X}_{\G, D^*_n}$ is positive.
For arbitrary $S$, we take a triangulation $T$ of $S$ and consider the triangles with the vertex at $p$. 
Go, if needed,  to a finite cover of $S$ to make sure that 
the triangles near $p$ form a polygon, providing an ideal triangulation of a punctured disc $D^*_n$. 
The action of the Weyl group affects only this polygon, and so it is positive.  Theorem \ref{13.5.4.11115h} is proved.








 

